Analysis of Sparse Recovery Algorithms via the Replica Method

This manuscript goes through the fundamental connections between statistical mechanics and estimation theory by focusing on the particular problem of compressive sensing. We first show that the asymptotic analysis of a sparse recovery algorithm is mathematically equivalent to the problem of calculating the free energy of a spin glass in the thermodynamic limit. We then use the replica method from statistical mechanics to evaluate the performance in the asymptotic regime. The asymptotic results have several applications in communications and signal processing. We briefly go through two instances of these applications: Characterization of joint sparse recovery algorithms used in distributed compressive sensing, and tuning of receivers employed for detection of spatially modulated signals.

==> commands.tex <==
\newcommand{\setX}{\mathbbmss{X}}
\newcommand{\setH}{\mathbbmss{H}}
\newcommand{\setL}{\mathbbmss{L}}
\newcommand{\setA}{\mathbbmss{A}}
\newcommand{\setP}{\mathbbmss{P}}
\newcommand{\setR}{\mathbbmss{R}}
\newcommand{\setV}{\mathbbmss{V}}
\newcommand{\setS}{\mathbbmss{S}}
\newcommand{\setW}{\mathbbmss{W}}
\newcommand{\setJ}{\mathbbmss{J}}
\newcommand{\setZ}{\mathbbmss{Z}}
\newcommand{\setB}{\mathbbmss{B}}
\newcommand{\setO}{\mathbbmss{O}}
\newcommand{\setC}{\mathbbmss{C}}
\newcommand{\setU}{\mathbbmss{U}}
\newcommand{\setT}{\mathbbmss{T}}

\DeclareMathOperator*{\argmin}{argmin} 
\DeclareMathOperator*{\argmax}{argmax} 


\newcommand{\rmP}{\Xi}
\newcommand{\ave}{\mathrm{P}}
\newcommand{\rmc}{\mathrm{c}}
\newcommand{\rmC}{\mathrm{C}}
\newcommand{\rmp}{\mathrm{p}}
\newcommand{\rmq}{\mathrm{q}}
\newcommand{\rmF}{\mathrm{F}}
\newcommand{\rmH}{\mathrm{H}}
\newcommand{\rmR}{\mathrm{R}}
\newcommand{\rmg}{\mathrm{g}}
\newcommand{\rmG}{\mathrm{G}}
\newcommand{\rmQ}{\mathrm{Q}}
\newcommand{\rmT}{\mathrm{T}}
\newcommand{\rmA}{\mathrm{A}}
\newcommand{\rmK}{\mathrm{K}}
\newcommand{\rmI}{\mathrm{I}}
\newcommand{\rmS}{\mathrm{S}}
\newcommand{\lams}{\lambda^{\mathsf{s}}}

\newcommand{\out}{\mathrm{out}}
\newcommand{\In}{\mathrm{in}}

\newcommand{\rsim}{\mathsf{Sim}^\mathsf{R}}
\newcommand{\her}{\mathsf{H}}

\newcommand{\sfF}{\mathsf{F}}
\newcommand{\sfI}{\mathsf{I}}
\newcommand{\sfT}{\mathsf{T}}
\newcommand{\sfC}{\mathsf{C}}
\newcommand{\sfM}{\mathsf{M}}
\newcommand{\sfQ}{\mathsf{Q}}
\newcommand{\sfE}{\mathsf{E}}
\newcommand{\sfD}{\mathsf{D}}
\newcommand{\sfW}{\mathsf{W}}
\newcommand{\sfr}{\mathsf{r}}
\newcommand{\sfR}{\mathsf{R}}
\newcommand{\sfd}{\mathsf{d}}
\newcommand{\sfZ}{\mathsf{Z}}
\newcommand{\sfL}{\mathsf{L}}
\newcommand{\sfK}{\mathsf{K}}
\newcommand{\sfp}{\mathsf{p}}
\newcommand{\sfa}{\mathsf{a}}


\newcommand{\mah}{\mathcal{H}}
\newcommand{\maf}{\mathcal{F}}
\newcommand{\mat}{\mathcal{T}}
\newcommand{\maP}{\mathcal{P}}
\newcommand{\mae}{\mathcal{E}}
\newcommand{\maz}{\mathcal{Z}}
\newcommand{\mas}{\mathcal{S}}
\newcommand{\mav}{\mathcal{V}}
\newcommand{\mab}{\mathcal{B}}
\newcommand{\man}{\mathcal{N}}
\newcommand{\mam}{\mathcal{M}}
\newcommand{\mad}{\mathcal{D}}
\newcommand{\mao}{\mathcal{O}}
\newcommand{\maq}{\mathcal{Q}}
\newcommand{\mg}{\mathcal{G}}
\newcommand{\mai}{\mathcal{I}}
\newcommand{\maj}{\mathcal{J}}
\newcommand{\mak}{\mathcal{K}}


\newcommand{\bxx}{\mathbf{x}}
\newcommand{\bi}{\mathbf{i}}
\newcommand{\bhxx}{\mathbf{x}}
\newcommand{\bss}{\mathbf{s}}
\newcommand{\bww}{\mathbf{w}}
\newcommand{\buu}{\mathbf{u}}
\newcommand{\bvv}{\mathbf{v}}
\newcommand{\byy}{\mathbf{y}}
\newcommand{\bgg}{\mathbf{g}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bhzz}{{\mathbf{z}}}

\newcommand{\snr}{P/ \sigma^2}

\newcommand{\rmx}{\mathrm{x}}
\newcommand{\rmj}{\mathrm{j}}
\newcommand{\rms}{\mathrm{s}}
\newcommand{\rmw}{\mathrm{w}}
\newcommand{\rmu}{\mathrm{u}}
\newcommand{\rmv}{\mathrm{v}}
\newcommand{\rmy}{\mathrm{y}}
\newcommand{\papr}{\mathrm{PAPR}}
\newcommand{\RLS}[2]{\mathrm{RLS}_{#1} \left( #2 \right)}
\newcommand{\rls}[2]{\mathrm{rls}_{#1} \left( #2 \right)}
\newcommand{\lse}{\mathrm{LSE}}
\newcommand{\dec}{\mathrm{dec}}
\newcommand{\reg}{\mathrm{reg}}
\newcommand{\loge}{\left. \mathrm{ln} \right.}
\newcommand{\sign}[1]{ \mathrm{sign} \left( #1 \right)}
\newcommand{\bh}{{\boldsymbol{h}}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bx}{{\boldsymbol{x}}}
\newcommand{\hx}{{\hat{x}}}
\newcommand{\tx}{{\tilde{x}}}
\newcommand{\tv}{{\tilde{v}}}
\newcommand{\hv}{{\hat{v}}}
\newcommand{\htt}{{\hat{t}}}
\newcommand{\vv}{\mathrm{v}}
\newcommand{\nn}{\mathrm{n}}
\newcommand{\hxx}{\hat{\mathrm{x}}}
\newcommand{\xx}{\mathrm{x}}
\newcommand{\yy}{\mathrm{y}}
\newcommand{\zz}{\mathrm{z}}
%\newcommand{\hxx}{\hat{\mathrm{x}}}
\newcommand{\btx}{\boldsymbol{\tilde{x}}}
\newcommand{\btv}{\boldsymbol{\tilde{v}}}
\newcommand{\bhx}{{\boldsymbol{\hat{x}}}}
\newcommand{\mar}{\mathcal{R}}
\newcommand{\mac}{\mathcal{C}}
%\newcommand{\repint}[1]{\mathfrak{S}^{\mu_{#1}}_{#1}}

\newcommand{\ty}{{\tilde{y}}}
\newcommand{\tz}{{\tilde{z}}}
\newcommand{\mfPt}{\tilde{\mathfrak{P}}}
\newcommand{\mfIt}{\tilde{\mathfrak{I}}}
\newcommand{\makt}{\tilde{\mathcal{K}}}

\newcommand{\bz}{{\boldsymbol{z}}}
\newcommand{\ba}{{\boldsymbol{a}}}
\newcommand{\bg}{{\boldsymbol{g}}}
\newcommand{\bs}{{\boldsymbol{s}}}
\newcommand{\br}{{\boldsymbol{r}}}
\newcommand{\bu}{{\boldsymbol{u}}}
\newcommand{\bv}{{\boldsymbol{v}}}
\newcommand{\bc}{{\boldsymbol{c}}}
\newcommand{\bw}{{\boldsymbol{w}}}

\newcommand{\pmf}{{\mathrm{P}}}
\newcommand{\pdf}{{\mathrm{f}}}
\newcommand{\cdf}{{\mathrm{F}}}


\newcommand{\bzz}{{\mathbf{z}}}
\newcommand{\baa}{{\mathbf{a}}}
\newcommand{\bdd}{{\mathbf{d}}}

\newcommand{\mfP}{\mathfrak{P}}
\newcommand{\mfI}{\mathfrak{I}}
\newcommand{\dif}{\mathrm{d}}

\newcommand{\by}{{\boldsymbol{y}}}
\newcommand{\hy}{{\hat{y}}}
\newcommand{\bhy}{{\boldsymbol{\hat{y}}}}

\newcommand{\bn}{{\boldsymbol{n}}}
\newcommand{\hn}{{\hat{n}}}
\newcommand{\be}{{\boldsymbol{e}}}

\newcommand{\trp}{\mathsf{T}}

\newcommand{\mA}{\mathbf{A}}
\newcommand{\mF}{\mathbf{F}}
\newcommand{\mR}{\mathbf{R}}
\newcommand{\ma}{\mathbf{A}}
\newcommand{\mI}{\mathbf{I}}
\newcommand{\mone}{\mathbf{1}}
\newcommand{\mJ}{\mathbf{J}}
\newcommand{\mG}{\mathbf{G}}
\newcommand{\mQ}{\mathbf{Q}}
\newcommand{\mS}{\mathbf{S}}
\newcommand{\mU}{\mathbf{U}}
\newcommand{\mGam}{\mathbf{A}}
\newcommand{\mD}{\mathbf{D}}
\newcommand{\mM}{\mathbf{M}}
\newcommand{\mLA}{\mathbf{\Lambda}}
\newcommand{\mX}{\mathbf{X}}
\newcommand{\mV}{\mathbf{V}}
\newcommand{\mtV}{\tilde{\mathbf{V}}}
\newcommand{\mB}{\mathbf{B}}
\newcommand{\mT}{\mathbf{T}}
\newcommand{\mH}{\mathbf{H}}

\newcommand{\rmE}{\mathrm{Erg}}


\newcommand{\md}{\mathrm{D}}
\newcommand{\E}{\mathsf{E}\hspace{.5mm}}
\newcommand{\MSE}{\mathsf{MSE}}
\newcommand{\mse}{\mathrm{MSE}}
\newcommand{\hp}{\hat{p}}
\newcommand{\rs}{{\mathsf{rs}}}
\newcommand{\rsb}{{\mathsf{rsb}}}
\newcommand{\asy}{{\mathrm{asy}}}



\newcommand{\C}{\mathbb{C}}

\newcommand{\Proofbegin}{\textbf{Proof.} }
\newcommand{\Proofend}{\hfill $.\square$ \\}
\newcommand{\discussion}{\textbf{Discussion.} }

\newcommand{\poster}[2]{\rmq_{\lams} ( #1 | #2 ) }

\newcommand{\Ex}[2]{\mathbbmss{E}_{#2}\left\{#1\right\}}
\newcommand{\norm}[1]{\lVert #1 \rVert}
\newcommand{\set}[1]{\left\lbrace #1 \right\rbrace}
\newcommand{\brc}[1]{\left( #1 \right)}
\newcommand{\dbc}[1]{\left[ #1 \right]}
\newcommand{\real}[1]{\mathbbm{Re}\left\lbrace #1 \right\rbrace}
\newcommand{\img}[1]{\mathbbm{Im}\left\lbrace #1 \right\rbrace}
\newcommand{\ind}[1]{\boldsymbol{1} \left\lbrace #1 \right\rbrace}
\newcommand{\abs}[1]{\lvert #1 \rvert}
\newcommand{\tr}[1]{\mathrm{Tr} \{ #1 \}}
\newcommand{\cosha}[1]{\mathrm{cosh}_{\alpha}\mathrm{(} #1 \mathrm{)}}
\newcommand{\pn}[1]{( #1 )}
\newcommand{\glse}[1]{\mathrm{glse}\left( #1 \right)}
\newcommand{\gred}[1]{\nabla_{\hspace*{-.5mm}#1} \hspace*{.5mm}}
\newcommand{\gredSq}[1]{\nabla^2_{\hspace*{-.5mm}#1} \hspace*{.5mm}}

\newcommand{\Sp}[1]{\mathrm{Supp}\left( #1 \right) }


\newcommand{\Tr}{\mathrm{Tr} }

%
\newtheoremstyle{mystyle}%                % Name
  {}%                                     % Space above
  {}%                                     % Space below
  {\it}%                                     % Body font
  {}%                                     % Indent amount
  {\bfseries}%                            % Theorem head font
  {:}%                                     % Punctuation after theorem head
  { }%                                    % Space after theorem head, ' ', or \newline
  {}%                                     % Theorem head spec (can be left empty, meaning `normal')

\theoremstyle{mystyle}


\renewcommand*{\proofname}{Sketch of the Proof}
\newtheorem{definition}{Definition}
\newtheorem{proposition}{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem{remark}{Remark}
\newtheorem*{prf}{Proof}
\newtheorem*{derivation}{Derivation}
\newtheorem*{tuning}{Tuning Approach}
%\newtheorem{theorem}{Theorem}[section]
\newtheorem{example}{Example}
%%\newtheorem{assumption}{Assumption}
%%\newtheorem{lemma}{Lemma}[section]
%%\newtheorem{remark}{Remark}[section]
%
%\renewenvironment{proof}{{\bfseries Proof. }}{\hfill$\blacktriangle$\vspace{2mm}}
%\declaretheorem[style=definition,qed=$\blacksquare$,numberwithin=section]{definition}
%\declaretheorem[style=proposition,qed=$\blacksquare$,numberwithin=section]{proposition}
%\declaretheorem[style=lemma,qed=$\blacksquare$,numberwithin=section]{lemma}
%\declaretheorem[style=assumption,qed=$\blacksquare$]{assumption}
%\declaretheorem[style=remark,numberwithin=section]{remark}
%
\algnewcommand\algorithmicLet{\textbf{Let}}
\algnewcommand\Let{\item[\algorithmicLet]}
%
\algnewcommand\algorithmicSet{\textbf{Set}}
\algnewcommand\Set{\item[\algorithmicSet]}


\algnewcommand\algorithmicInitiate{\textbf{Initiate}}
\algnewcommand\Initiate{\item[\algorithmicInitiate]}
%
\algnewcommand\algorithmicStart{\textbf{Begin}}
\algnewcommand\Begin{\item[\algorithmicStart]}
%
\algnewcommand\algorithmicEnd{\textbf{End}}
\algnewcommand\End{\item[\algorithmicEnd]}

\algnewcommand\algorithmicOutP{\textbf{Output:}}
\algnewcommand\Out{\item[\algorithmicOutP]}
%\algnewcommand\algorithmicimplement{\textbf{implement}}
%\algnewcommand\Implement{\item[\algorithmicimplement]}
%
%\algnewcommand\algorithmicbegin{\textbf{begin}}
%\algnewcommand\BEGIN{\item[\algorithmicbegin]}
%
\newcommand\NoDo{\renewcommand\algorithmicdo{}}
%\algnewcommand\algorithmicEnd{\textbf{end}}
%\algnewcommand\ENDall{\item[\algorithmicEnd]}
%
%\algnewcommand\algorithmicoutput{\textbf{output}}
%\algnewcommand\Output{\item[\algorithmicoutput]}

\newcounter{bar}
\newcommand{\exmpl}[1]{\refstepcounter{bar}\label{#1} \textbf{Example \thebar. }}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\mj}{\mathrm{J}}
\newcommand{\mtX}{\mathrm{\tilde{X}}}
\newcommand{\mt}{\mathrm{T}}
%\newcommand{\tx}{{\tilde{x}}}
%\newcommand{\btx}{\boldsymbol{\tilde{x}}}
